Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly

Self-assembly refers to the process by which small, simple components mix and combine to form complex structures using only local interactions. Designed as a hybrid between tile assembly models and cellular automata, the Tile Automata (TA) model was recently introduced as a platform to help study connections between various models of self-assembly. However, in this paper we present a result in which we use TA to simulate arbitrary systems within the amoebot model, a theoretical model of programmable matter in which the individual components are relatively simple state machines that are able to sense the states of their neighbors and to move via series of expansions and contractions. We show that for every amoebot system, there is a TA system capable of simulating the local information transmission built into amoebot particles, and that the TA "macrotiles" used to simulate its particles are capable of simulating movement (via attachment and detachment operations) while maintaining the necessary properties of amoebot particle systems. The TA systems are able to utilize only the local interactions of state changes and binding and unbinding along tile edges, but are able to fully simulate the dynamics of these programmable matter systems.

==> DNA25-acceptance-and-reviews.tex <==
Reviewer comments/suggestions:

- [DONE (MJP): Add an acknowledgement for the Dagstuhl seminar]

-----------
Reviewer 1:
-----------
- [DONE (MJP: added a paragraph near the end of the intro which hopefully provides more motivation.): maybe add a bit more motivation text to the second to last paragraph of the intro] It would be great if the authors could show some unique advantage of TA model in modeling programmable matter.

-----------
Reviewer 2:
-----------
- [IGNORE(?): this result would not imply power of amoebots, but instead of TA. The reviewer seems to have it backward, and I don't think this comment needs to be addressed] it would  be useful to add some comments regarding the implications of this result.  What does this simulation result imply, regarding the computational power of amoebot systems? (As TA is a new model which differs from TAM in several ways, I do not know off the top of my head  many characterizations  of  TA's computational power.) 

- [DONE (MJP: added a paragraph near the end of the intro which hopefully provides more motivation.): additional motivating text in the intro should help with this, too.]  Alternatively, if comparisons  or the equivalence of computational power are not the driving goal, then what other goals and consequences does this  simulation have?

-----------
Reviewer 3:
-----------
- [TODO: depending on space allowance, we can consider adding another figure or two] I think this paper would greatly benefit from more diagrams, as the whole operation of this TA is very complicated and consists of many stages. I have to admit that I had a lot of difficulty following exactly how this TA will carry out each operation. 

- [TODO: maybe try to add a figure showing an ``animation'' of a portion of the process] The diagram in Figure 5 is very helpful, but I am still perplexed trying to use my imagination for how the signals will propagate in the right directions on the tile assembly when the timing tile pops into place. For example, where is the flag displayed on the tile? I would have liked to have a bigger diagram explaining how the clock part works, as it also has quite a few moving parts that have to work together.

- [DONE: maybe add a bit more detail in the caption. This reviewer seems to be quite confused, as this is not an illustration of a handover.] In Figure 6, we see three stages of a handover operation, which is also helpful to illustrate, but it is still not shown in quite enough granularity for me to fully follow. There are lot of little details that are going on that are confusing, such as the little timing tiles appearing and disappearing, they are doing something, but I don't fully understand how they move around.  I realize you are trying to find a balance between fully labelling 100 mini sub tiles... but some more labels would help.

- [IGNORE (for now): it would be great to have an illustration showing each step, but that would remain in an appendix and therefore not be in the proceedings. Perhaps for an arxiv version and possible journal version.] The example turn C1 at the end was actually the most useful section for me to try and understand how this is all working together, but this would also benifit from also being illustrated showing the state of the TA at each of these 16 steps.

- [DONE?: Make sure the description of R is clear enough.] Lastly, the Configuration Tile seems to be the most limiting factor in actually realizing this in DNA. I know that's a while off still.. But let's just think about how fancy this tile has to be: This tile has to somehow function as the amoebot's sense of self-awareness, and combine all the signalling information from all the surrounding tiles back into itself in some physical manner. At the end of the turn it combines all the different signal information from multiple surrounding tiles into a single place, even if the signals are just little tiny pieces of DNA we've got a whole bunch of those combining all at once in this step.  I think it would help if you could spell out in more detail how "the configuration tile is used by the representation function R to map the active macrotile to its previous configuration".

-----------
Reviewer 4:
-----------
- [IGNORE: I don't really think that would simplify things much, and would require a massive reworking of the construction and proof.] General comment, I am not sure why one has to use square tiles for the simulation. The macro tiles a[re] hexagonal and they have 100 square tiles to allow no interactions between the signals passed between neighboring pairs of tiles. One can use hexagonal tiles that as dual tile the triangular lattice,  then equip these tiles with the same signals and state transition properties according to their neighboring glues.  It seems the simulation would be much simpler, and more straight forward. Then, if one wants to use square tiles, one only needs to show that the hexagonal tiles can be simulated. 
Since there is no description of a DNA system that can implement the tile automata, one can as well take hexagonal tiles vs squares. 

- [DONE: add a brief mention of why the triangular lattice is preferred for amoebots in the definition of the model.] Or vice versa, what can amoebot system achieve on a triangular lattice that cannot be achieved on a square lattice? In fact one can consider any periodic lattice in a plane as the underlined graph.

- [DONE: add space between the squares.] In Fig. 1 it seems the squares in the  box labeled `states’ should be separated. 

- [DONE(?): maybe remove use of [i] notation (given at the bottom of page 4) and instead use {0,1,2,3,4,5} and {0,1,2,3,4,5,6,7,8,9} in place of [5] and [9], respectively.] The notation [9] and [5] is often confused with a notation for a citation. Maybe use a set J as an index set. 

- [DONE: define a ``particle system'' simply as a group of particles(?). However, I do think that ``initial configuration'' is defined: ``the initial system configuration of \mathcal{A} mapping each particle to its starting configuration''.] On page 7: `particle system’ is not defined, also `initial configuration’ is not defined. 

- [DONE: OOPS! Stupid mistake! Fix this!! ]Page 9: Definitions should refer to Tile Automata Systems

-----------
Reviewer 5:
-----------
- [DONE: It would be worth discussing if growth and dissolution of floats could be easily done instead.] For the simulation of movement, in particular the expansion I wonder why the authors chose to use floating macrotiles? Another option would be to merely self-assemble the expanded macrotile; which seems more straightforward. I might have missed a piece of the text explaining this?

- [DONE (MJP): Good call! Added citation to \cite{IUSA} and others and a blurb about how these are ``standard'' definitions in other papers.] Section 4 should cite previous self-assembly papers that defined "models", "follows", and "simulates", in order (a) recognize that the definitions here borrow from previous work and (b) to help the reader know which previous definitions are used (there are a number of previous defs, and it could be confusing for someone to navigate both this paper and that previous literature). 

- [DONE] abstract:
  between varying models of self-assembly. ->
  between various models of self-assembly.



===========================================================================
===========================================================================
Following is the complete DNA 25 acceptance email with full reviews:
--------------------------------------------------------------------

On behalf of the DNA25 program committee we are pleased to inform you that your Track A submission

Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly

has been selected for oral presentation at DNA25 and for publication in the LNCS proceedings of the conference.

The reviews are enclosed. Please take them into careful consideration when preparing your revised manuscript.  The final version is due on June 21, 2019.  Due to the timing of this year's conference, there is *no flexibility in this due date*.  Please plan accordingly as final manuscripts not submitted by the deadline risk being left out of this year's proceedings.

Detailed instructions for preparing the LNCS final version of your paper will be sent in a separate email.

At least one author must register and be prepared to present at the conference.  To register for the conference and reserve accommodation please visit http://misl.cs.washington.edu/events/dna25/. Early registration ends on June 30. A limited number of discounted hotel rooms and on campus options are available.

We look forward to seeing you at DNA25 in Seattle!

With congratulations,
Yan Liu and Chris Thachuk
DNA 25 Program Committee Co-Chairs

SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly


----------------------- REVIEW 1 ---------------------
SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly
AUTHORS: John Alumbaugh, Joshua Daymude, Erik Demaine, Matthew Patitz and Andrea Richa

----------- Overall evaluation -----------
SCORE: 5 (accept)
----------- Review -----------
This paper shows how to use Tile Automata (TA) model to simulate arbitrary systems in the amoebot model (an abstract model of programmable matter). The constructions look correct. Besides solving theoretical problems, this work also suggests potential usefulness of TA model in material science.  It would be great if the authors could show some unique advantage of TA model in modeling programmable matter.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly
AUTHORS: John Alumbaugh, Joshua Daymude, Erik Demaine, Matthew Patitz and Andrea Richa

----------- Overall evaluation -----------
SCORE: 5 (accept)
----------- Review -----------
This paper  makes a connection between a self-assembly model and  programmable matter model. In particular, the authors show  that the Tile Automata (TA) model can be used to simulate the amoebot model (wherein "particles" solve problems  such as shape formation, object coating, leader election, gathering, bridging gaps, etc., by using  strictly local information and communication). The simulation  is obtained by a construction whereby "macrotiles"  are able to simulate the behaviour of individual amoebot particles, and  are able to  collectively simulate the dynamics of amoebot systems.

I found that this paper makes a very  interesting connection  between two different  computational models.  In the long term, it would be useful to see a software simulation of how the TA system that models the amoebot system works in practice. In the short term, for this paper, it would  be useful to add some comments regarding the implications of this result.  What does this simulation result imply, regarding the computational power of amoebot systems? (As TA is a new model which differs from TAM in several ways, I do not know off the top of my head  many characterizations  of  TA's computational power. ) Alternatively, if comparisons  or the equivalence of computational power are not the driving goal, then what other goals and consequences does this  simulation have?

Overall, I think this paper would be of great interest to the conference participants, and I recommend it for acceptance.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly
AUTHORS: John Alumbaugh, Joshua Daymude, Erik Demaine, Matthew Patitz and Andrea Richa

----------- Overall evaluation -----------
SCORE: 5 (accept)
----------- Review -----------
The authors have taken the abstract Amoebot Model and devised a way to simulate that complex behavior using a Tile Automata model. This is a very fascinating representation, where each amoebot is modeled as a network of assembled macrotiles that work together as a little processing node with a 'clock'. I think that this would be of particular interest to the DNA25 conference as it fits in the overall theme of this conference exploring all avenues of different computational systems that might be potentially implemented experimentally. The idea is interesting and well thought out. I suggest that we accept this paper for the conference.


I think this paper would greatly benefit from more diagrams, as the whole operation of this TA is very complicated and consists of many stages. I have to admit that I had a lot of difficulty following exactly how this TA will carry out each operation. 

The diagram in Figure 5 is very helpful, but I am still perplexed trying to use my imagination for how the signals will propagate in the right directions on the tile assembly when the timing tile pops into place. For example, where is the flag displayed on the tile? I would have liked to have a bigger diagram explaining how the clock part works, as it also has quite a few moving parts that have to work together.

In Figure 6, we see three stages of a handover operation, which is also helpful to illustrate, but it is still not shown in quite enough granularity for me to fully follow. There are lot of little details that are going on that are confusing, such as the little timing tiles appearing and disappearing, they are doing something, but I don't fully understand how they move around.  I realize you are trying to find a balance between fully labelling 100 mini sub tiles... but some more labels would help.

The example turn C1 at the end was actually the most useful section for me to try and understand how this is all working together, but this would also benifit from also being illustrated showing the state of the TA at each of these 16 steps.

Lastly, the Configuration Tile seems to be the most limiting factor in actually realizing this in DNA. I know that's a while off still.. But let's just think about how fancy this tile has to be: This tile has to somehow function as the amoebot's sense of self-awareness, and combine all the signalling information from all the surrounding tiles back into itself in some physical manner. At the end of the turn it combines all the different signal information from multiple surrounding tiles into a single place, even if the signals are just little tiny pieces of DNA we've got a whole bunch of those combining all at once in this step.  I think it would help if you could spell out in more detail how "the configuration tile is used by the representation function R to map the active macrotile to its previous configuration".



----------------------- REVIEW 4 ---------------------
SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly
AUTHORS: John Alumbaugh, Joshua Daymude, Erik Demaine, Matthew Patitz and Andrea Richa

----------- Overall evaluation -----------
SCORE: 4 (weak accept)
----------- Review -----------
The paper considers two models: Tile Automata Model and Amoebot Model. The former is a variant of a 2HAM model equipped with signals where it is assumed that the tiles are equipped with a transition function such that when two tiles attached, the signal system can change their pair of states according to a predefined transition function. The Amoebot Model is a model that consists of a set of `particles’ that populate the triangular lattice. Each particle can be contracted (just a vertex) or it can be expanded to be two vertices connected with an edge of the lattice, in which case one of the vertices is a head and the other is a tail. The particles act as automata (with a local transition function) such that they `decide’ on their next move according to the states of the neighboring particles. The neighborhood has at most 6 vertices when the particle is contracted, and has at most ten vertices when the particle is expanded. At each configuration at most 2n vertices are populated of the lattice when there are n particles. The system changes by choosing a particle and changing its state according to the local function. 

The paper simulates the Amoebot Model with a Tile Automata Model. Although there are details of the simulation to be worked out, the simulation seems to be straight forward. Each vertex of the triangular lattice is associated to  a macro tile of 100 square units that have hexagonal shape and the state of the tiles in the center indicate what type of vertex of the Amoebot system they represent. The transition function of the square tiles can be tweaked to pass signals to the neighboring macro tile in the same way as the particles check their neighbors, and change their states.

General comment, I am not sure why one has to use square tiles for the simulation. The macro tiles a hexagonal and they have 100 square tiles to allow no interactions between the signals passed between neighboring pairs of tiles. One can use hexagonal tiles that as dual tile the triangular lattice,  then equip these tiles with the same signals and state transition properties according to their neighboring glues.  It seems the simulation would be much simpler, and more straight forward. Then, if one wants to use square tiles, one only needs to show that the hexagonal tiles can be simulated. 
Since there is no description of a DNA system that can implement the tile automata, one can as well take hexagonal tiles vs squares. 

Or vice versa, what can amoebot system achieve on a triangular lattice that cannot be achieved on a square lattice? In fact one can consider any periodic lattice in a plane as the underlined graph.

Some more detailed comments:

In Fig. 1 it seems the squares in the  box labeled `states’ should be separated. 

The notation [9] and [5] is often confused with a notation for a citation. Maybe use a set J as an index set. 

On page 7: `particle system’ is not defined, also `initial configuration’ is not defined. 

Page 9: Definitions should refer to Tile Automata Systems



----------------------- REVIEW 5 ---------------------
SUBMISSION: 27
TITLE: Simulation of Programmable Matter Systems Using Active Tile-Based Self-Assembly
AUTHORS: John Alumbaugh, Joshua Daymude, Erik Demaine, Matthew Patitz and Andrea Richa

----------- Overall evaluation -----------
SCORE: 4 (weak accept)
----------- Review -----------
The paper is on the topic of simulation between the Tile Automata model and the Amoebot model. Both are active models, in these sense that given tiles/amoebot units can change their state. Both models are asynchronous cellular automata. Since simulation has been used to compare a range of self-assembly models, and gives definitions equipped to handle tricky timing/asynchronicity issues this seems a great tool to compare models and to understand where Amoebots fits in the theory of self-assembly universe. 

Opinion:

Overall the paper is perhaps useful to the community as it points out how these models are similar, and how to think about amoebots in a self-assembly setting.

Indeed much of the proof is concerned with handling the asynchronicity of Amoebots in the scaled-up and asynchronous TA setting. 

For the simulation of movement, in particular the expansion I wonder why the authors chose to use floating macrotiles? Another option would be to merely self-assemble the expanded macrotile; which seems more straightforward. I might have missed a piece of the text explaining this?

Minor:

Section 4 should cite previous self-assembly papers that defined "models", "follows", and "simulates", in order (a) recognize that the definitions here borrow from previous work and (b) to help the reader know which previous definitions are used (there are a number of previous defs, and it could be confusing for someone to navigate both this paper and that previous literature). 

abstract:
between varying models of self-assembly. ->
between various models of self-assembly.

==> oldBibList.tex <==



\begin{thebibliography}{}

\bibitem{amoebots}
Zahra Derakhshandeh, Shlomi Dolev, Robert Gmyr, Andréa W. Richa, Christian
Scheideler, and Thim Strothmann. ``Brief announcement: Amoebot — a new model for programmable matter." In SPAA, 2014.

\bibitem{freezing}
Chalk, Cameron, et al. ``Freezing Simulates Non-freezing Tile Automata." International Conference on DNA Computing and Molecular Programming. Springer, Cham, 2018.

\bibitem{smartPart}
Cannon, Sarah, et al. ``A Markov chain algorithm for compression in self-organizing particle systems." Proceedings of the 2016 ACM Symposium on Principles of Distributed Computing. ACM, 2016.

\bibitem{STAM}Keenan, Alexandra, Robert Schweller, and Xingsi Zhong. ``Exponential replication of patterns in the signal tile assembly model." International Workshop on DNA-Based Computers. Springer, Cham, 2013.

\bibitem{graphlets}Alumbaugh, John Calvin, Qinghua Li, and Vincent Hu.``Differentiating Non-Isomorphic Graphlets for Graph Analytics." Collaboration and Internet Computing (CIC), 2016 IEEE 2nd International Conference on. IEEE, 2016.

\end{thebibliography}
